Causal Structural Learning on MPHIA Individual Dataset

The Population-based HIV Impact Assessment (PHIA) is an ongoing project that conducts nationally representative HIV-focused surveys for measuring national and regional progress toward UNAIDS' 90-90-90 targets, the primary strategy to end the HIV epidemic. We believe the PHIA survey offers a unique opportunity to better understand the key factors that drive the HIV epidemics in the most affected countries in sub-Saharan Africa. In this article, we propose a novel causal structural learning algorithm to discover important covariates and potential causal pathways for 90-90-90 targets. Existing constrained-based causal structural learning algorithms are quite aggressive in edge removal. The proposed algorithm preserves more information about important features and potential causal pathways. It is applied to the Malawi PHIA (MPHIA) data set and leads to interesting results. For example, it discovers age and condom usage to be important for female HIV awareness; the number of sexual partners to be important for male HIV awareness; and knowing the travel time to HIV care facilities leads to a higher chance of being treated for both females and males. We further compare and validate the proposed algorithm using BIC and using Monte Carlo simulations, and show that the proposed algorithm achieves improvement in true positive rates in important feature discovery over existing algorithms.

==> tables/AIC.tex <==
% Generated by SimulationTables: do not edit by hand

\begin{table}[!ht]
\caption{\label{tab:IC}Comparison of different graphical learning methods by Bayesian Information Criterion. Aware, ART, and VLS stand for the three 90-90-90 targets of HIV awareness, ART treatment, and viral load suppression respectively. DF stands for the number of degree of freedom.
Log-likelihood* is the difference between the log-likelihood and the log-likelihood of the null model (model with intercept only).}
% AIC is $-2\text{Log-likelihood*} + 2\text{DF}$, and BIC is $-2\text{Log-likelihood*} + \text{DF} \log(n)$, where $n$ is the sample size.
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}[t]{llrrrrrrrr}
\toprule
\multicolumn{2}{c}{ } & \multicolumn{4}{c}{Male} & \multicolumn{4}{c}{Female} \\
\cmidrule(l{3pt}r{3pt}){3-6} \cmidrule(l{3pt}r{3pt}){7-10}
Goals & Method & DF & Log-likelihood* & AIC & BIC & DF & Log-likelihood* & AIC & BIC\\
\midrule
 & PC-stable & 18 & 845.2 & -1,654.3 & -1,572.1 & 0 & 0.0 & 0.0 & 0.0\\

 & MMPC & 20 & 736.6 & -1,433.1 & -1,341.8 & 100 & 10,541.6 & -20,883.2 & -20,351.5\\

 & IAMB & 20 & 736.6 & -1,433.1 & -1,341.8 & 118 & 13,041.9 & -25,847.9 & -25,220.5\\

 & GS & 81 & 2,348.3 & -4,534.7 & -4,164.7 & 69 & 6,027.7 & -11,917.5 & -11,550.6\\

\multirow{-5}{*}{\raggedright\arraybackslash Aware} & New & 948 & 17,896.1 & -33,896.2 & -29,565.7 & 1,021 & 53,416.3 & -104,790.6 & -99,362.4\\
\cmidrule{1-10}
 & PC-stable & 6 & 183.6 & -355.2 & -329.8 & 8 & 690.0 & -1,363.9 & -1,323.1\\

 & MMPC & 8 & 341.5 & -667.1 & -633.2 & 92 & 8,388.6 & -16,593.1 & -16,124.1\\

 & IAMB & 8 & 341.5 & -667.1 & -633.2 & 108 & 9,854.8 & -19,493.7 & -18,943.0\\

 & GS & 62 & 1,573.6 & -3,023.2 & -2,760.7 & 96 & 6,712.0 & -13,232.0 & -12,742.5\\

\multirow{-5}{*}{\raggedright\arraybackslash ART} & New & 974 & 10,460.6 & -18,973.2 & -14,848.9 & 2,127 & 49,249.3 & -94,244.7 & -83,400.4\\
\cmidrule{1-10}
 & PC-stable & 6 & 162.4 & -312.8 & -288.1 & 4 & 289.4 & -570.9 & -550.8\\

 & MMPC & 8 & 303.1 & -590.3 & -557.3 & 116 & 9,553.3 & -18,874.6 & -18,293.2\\

 & IAMB & 8 & 303.1 & -590.3 & -557.3 & 108 & 9,379.4 & -18,542.9 & -18,001.6\\

 & GS & 63 & 1,888.7 & -3,651.5 & -3,392.0 & 104 & 6,074.3 & -11,940.5 & -11,419.3\\

\multirow{-5}{*}{\raggedright\arraybackslash VLS} & New & 1,151 & 9,241.6 & -16,181.2 & -11,441.3 & 983 & 43,096.9 & -84,227.8 & -79,300.9\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/node_edge_legend.tex <==
% Generated by SimulationTables: do not edit by hand

%%\begin{table}[H]
\centering\begingroup\fontsize{8}{10}\selectfont

\begin{tabular}[t]{l>{}ll>{}l}
	\toprule
	Node &   & Edge significance &  \\
	\midrule
	90-90-90 Target & \includegraphics[width=0.67in, height=0.17in]{./figures/node_1.pdf} & $<0.001$ & \includegraphics[width=0.67in, height=0.17in]{./figures/edge_1.pdf}\\
	Neighbor of Target & \includegraphics[width=0.67in, height=0.17in]{./figures/node_2.pdf} & $<0.01$ & \includegraphics[width=0.67in, height=0.17in]{./figures/edge_2.pdf}\\
	Neighbor of Neighbor & \includegraphics[width=0.67in, height=0.17in]{./figures/node_3.pdf} & $<0.05$ & \includegraphics[width=0.67in, height=0.17in]{./figures/edge_3.pdf}\\
	\bottomrule
\end{tabular}
\endgroup{}
%% \end{table}

